Network-Controlled Repeaters vs. Reconfigurable Intelligent Surfaces for 6G mmW Coverage Extension

Network-controlled repeaters (NCR) and reconfigurable intelligent surfaces (RIS) are being considered by the third generation partnership project (3GPP) as valid candidates for range extension in millimeter-wave (mmW, 30-300 GHz frequency) 5G and 6G networks, to counteract large path and penetration losses. Nowadays, there is no definite answer on which of the two technologies is better for coverage extension, since existing comparative studies focused either on communication-related metrics only or on very large-scale analysis, without physical layer details or environmental considerations. This paper aims at comparing NCR and RIS solutions in terms of coverage in an urban scenario. Numerical results suggest a possible usage of both technologies, showing that preferring RIS or NCR depends not only on their physical capabilities and cost (e.g., the number of antenna elements, the angular separation between panels for NCR, etc.) but also on environment geometry.

==> Article - RIS vs AF/packages.tex <==
\usepackage{xcolor}
\usepackage{cite}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage[short]{optidef}
%\usepackage{subfig}
%\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{mwe}
\usepackage{url}
%\usepackage[pdftex]{graphicx}
%\usepackage{comment}
%\usepackage{easyReview}
%\usepackage{autobreak}
\usepackage{glossaries-extra}
\setabbreviationstyle[acronym]{long-short}
\newacronym{RIS}{RIS}{reconfigurable intelligent surface}

\newacronym{mmW}{mmW}{millimeter-wave, 30-300 GHz frequency}

\newacronym{THz}{THz}{terahertz}
\newacronym{SNR}{SNR}{signal-to-noise ratio}
\newacronym{UE}{UE}{user equipment}
\newacronym{AF}{AF}{amplify and forward}
\newacronym{FoV}{FoV}{field of view}

\newacronym{NCR}{NCR}{Network-controlled repeater}

\newacronym{DF}{DF}{decode and forward}

\newacronym{SRE}{SRE}{smart radio environment}

\newacronym{SR}{SR}{smart repeaters}

\newacronym{BS}{BS}{base station}

\newacronym{AoD}{AoD}{angle of departure}

\newacronym{E2E}{E2E}{end-to-end}


==> packages.tex <==
\usepackage{xcolor}
\usepackage{cite}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage[short]{optidef}
%\usepackage{subfig}
%\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{mwe}
\usepackage{url}
%\usepackage[pdftex]{graphicx}
%\usepackage{comment}
%\usepackage{easyReview}
%\usepackage{autobreak}
\usepackage{glossaries-extra}
\setabbreviationstyle[acronym]{long-short}
\newacronym{RIS}{RIS}{reconfigurable intelligent surface}

\newacronym{mmW}{mmW}{millimeter-wave, 30-300 GHz frequency}

\newacronym{THz}{THz}{terahertz}
\newacronym{SNR}{SNR}{signal-to-noise ratio}
\newacronym{UE}{UE}{user equipment}
\newacronym{AF}{AF}{amplify and forward}
\newacronym{FoV}{FoV}{field of view}

\newacronym{NCR}{NCR}{Network-controlled repeater}

\newacronym{DF}{DF}{decode and forward}

\newacronym{SRE}{SRE}{smart radio environment}

\newacronym{SR}{SR}{smart repeaters}

\newacronym{BS}{BS}{base station}

\newacronym{AoD}{AoD}{angle of departure}

\newacronym{E2E}{E2E}{end-to-end}

